Study of the kinematic dependences of $\Lambda_b^0$ production in $pp$ collisions and a measurement of the $\Lambda_b^0 \rightarrow \Lambda_c^+ \pi^-$ branching fraction

The kinematic dependences of the relative production rates, $f_{\Lambda_b^0}/f_d$, of $\Lambda_b^0$ baryons and $\bar{B}^0$ mesons are measured using $\Lambda_b^0 \rightarrow \Lambda_c^+ \pi^-$ and $\bar{B}^0 \rightarrow D^+ \pi^-$ decays. The measurements use proton-proton collision data, corresponding to an integrated luminosity of 1 fb$^{-1}$ at a centre-of-mass energy of 7 TeV, recorded in the forward region with the LHCb experiment. The relative production rates are observed to depend on the transverse momentum, $p_T$, and pseudorapidity, $\eta$, of the beauty hadron, in the studied kinematic region $1.5 < p_T < 40$ GeV/$c$ and $2 < \eta < 5$. Using a previous LHCb measurement of $f_{\Lambda_b^0}/f_d$ in semileptonic decays, the branching fraction $\mathcal{B}(\Lambda_b^0 \rightarrow \Lambda_c^+ \pi^-) = \Big( 4.30 \pm 0.03 \,\, ^{+0.12}_{-0.11} \pm 0.26 \pm 0.21 \Big) \times 10^{-3}$ is obtained, where the first uncertainty is statistical, the second is systematic, the third is from the previous LHCb measurement of $f_{\Lambda_b^0}/f_d$ and the fourth is due to the $\bar{B}^0 \rightarrow D^+ \pi^-$ branching fraction. This is the most precise measurement of a $\Lambda_b^0$ branching fraction to date.

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 18784 2012-04-30 14:45:53Z uegede $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}

